Voice Biomarker Analysis and Automated Severity Classification of Dysarthric Speech in a Multilingual Context

Dysarthria, a motor speech disorder, severely impacts voice quality, pronunciation, and prosody, leading to diminished speech intelligibility and reduced quality of life. Accurate assessment is crucial for effective treatment, but traditional perceptual assessments are limited by their subjectivity and resource intensity. To mitigate the limitations, automatic dysarthric speech assessment methods have been proposed to support clinicians on their decision-making. While these methods have shown promising results, most research has focused on monolingual environments. However, multilingual approaches are necessary to address the global burden of dysarthria and ensure equitable access to accurate diagnosis. This thesis proposes a novel multilingual dysarthria severity classification method, by analyzing three languages: English, Korean, and Tamil.

==> figures/3_alignment.tex <==
\begin{table}[h]
\captionsetup{justification=centering}
\caption{Alignment for phoneme correctness extraction. Correctly recognized phonemes are indicated in bold. * in canonical phoneme sequence and decoded phoneme sequence each indicates deletion and insertion.}
\label{tab:alignment}
\centering
\resizebox{0.50\textwidth}{!}{
\begin{tabular}{c}
\hline\hline
Canonical phoneme sequence \\
\hline
HH  \textbf{IY}  \textbf{W}  IH  \textbf{L}  \textbf{AH}  \textbf{L}  \textbf{AW}  AH  *  R  EH  L  \textbf{AY} \\
\hline
\hline
Decoded phoneme sequence \\
\hline
SH  \textbf{IY}  \textbf{W}  AO  \textbf{L}  \textbf{AH}  \textbf{L}  \textbf{AW}  AE  N  L  IY  *  \textbf{AY}\\
\hline
\hline
\end{tabular}
}
\end{table}

==> figures/3_features_tbl.tex <==
\begin{table*}[h]
\caption{Acoustic features}
\label{tab:acoustic features}
\centering

\resizebox{0.98\textwidth}{!}{%
\begin{tabular}{c|c|c}

\hline
\multicolumn{2}{c|}{Category} & Features \\

\hline
\multicolumn{2}{c|}{Voice quality} & jitter, shimmer, PPQ, APQ, HNR, number of voice breaks, degree of voice breaks \\
\hline

% \hline
% \multirow{2}{*}{Voice quality} & Glottal flow & jitter, shimmer, PPQ, APQ, HNR \\
% \cline{2-3}
% & Phonation & \# of voice breaks, \% of voice breaks \\
% \hline

\multirow{2}{*}{Pronunciation} & Phoneme correctness & PCC, PCV, PCP \\
\cline{2-3}
& Vowel distortion & triangular VSA, quadrilateral VSA, FCR, VAI, F2-Ratio \\
\hline

\multirow{5}{*}{Prosody} 
& Speech rate & speaking rate, articulation rate, number of pauses, pause duration, phone ratio \\
\cline{2-3}
& Pitch & mean, std, min, max, range of F0 \\
\cline{2-3}
& Loudness & mean, std, min, max, range of energy \\
\cline{2-3}
& Rhythm & \%V, deltaV/C, VarcoV/C, rPVIV/C, nPVIV/C \\
\cline{2-3}
\hline

\end{tabular}%
}
\end{table*}

==> figures/5_english_importance.tex <==
\begin{table}[htbp]
\centering
\caption{Feature Importance (English)}
\label{tab:feature_importance}
\begin{tabular}{lllr}
\toprule
\textbf{Features} & \textbf{Feature Type} & \textbf{Feature Subtype} & \textbf{Importance} \\
\midrule
Maximum energy                 & prosody        & energy            & 0.0723 \\
CRR             & pronunciation  & phoneme accuracy  & 0.0615 \\
Minimum energy                & prosody        & energy            & 0.0575 \\
PRR                    & pronunciation  & phoneme accuracy  & 0.0530 \\
\%V                       & prosody        & rhythm            & 0.0522 \\
PPQ                & voice quality  & voice quality     & 0.0509 \\
speaking rate             & prosody        & fluency           & 0.0468 \\
Median F0                 & prosody        & F0                & 0.0463 \\
VarcoC                    & prosody        & rhythm            & 0.0448 \\
VAI                       & pronunciation  & vowel distortion  & 0.0427 \\
VRR           & pronunciation  & phoneme accuracy  & 0.0422 \\
VSA$\triangle$                   & pronunciation  & vowel distortion  & 0.0419 \\
articulation rate        & prosody        & fluency           & 0.0413 \\
nPVIV                    & prosody        & rhythm            & 0.0403 \\
Maximum F0                 & prosody        & F0                & 0.0395 \\
average pause dur.       & prosody        & fluency           & 0.0394 \\
F2-Ratio                        & pronunciation  & vowel distortion  & 0.0393 \\

\# of pauses               & prosody        & fluency           & 0.0391 \\
VSA$\square$                      & pronunciation  & vowel distortion  & 0.0390 \\
percentage of vb.                     & voice quality  & voice quality     & 0.0389 \\
FCR                       & pronunciation  & vowel distortion  & 0.0361 \\
\# of vb.                       & voice quality  & voice quality     & 0.0352 \\
\bottomrule
\end{tabular}
\end{table}

==> figures/5_english_multivariate.tex <==
\begin{table}[htbp]
\centering
\caption{Multivariate Regression Results for Dysarthria Severity}
\label{tab:regression_results}
\begin{tabular}{lcccc}
\toprule
\textbf{Feature} & \textbf{Coefficient} & \textbf{Std. Error} & \textbf{t-value} & \textbf{p-value} \\
\midrule
ppq5Jitter          & 22.3345 & 4.601 & 4.855 & 0.000 \\
EMinimum            & -24.6001 & 6.568 & -3.745 & 0.000 \\
EMaximum            & 1.2699 & 0.161 & 7.898 & 0.000 \\
VAI                 & 3.9302 & 1.775 & 2.214 & 0.027 \\
FCR                 & 3.0201 & 0.891 & 3.390 & 0.001 \\
F2                  & 0.5240 & 0.156 & 3.349 & 0.001 \\
const               & -5.5588 & 2.473 & -2.247 & 0.025 \\
PMaximum            & 0.0013 & 0.000 & 3.768 & 0.000 \\
$\%V$.                 & 1.1020 & 0.562 & 1.962 & 0.050 \\
articulation_rate   & -0.0842 & 0.033 & -2.553 & 0.011 \\
nPVI-V              & -0.0459 & 0.008 & -5.814 & 0.000 \\
VSA1                & -1.071e-06 & 6.43e-07 & -1.666 & 0.096 \\
VSA2                & -5.173e-07 & 4.58e-07 & -1.130 & 0.259 \\
PCP                 & -1.0146 & 1.078 & -0.941 & 0.347 \\
PMediman            & -0.0009 & 0.001 & -1.434 & 0.152 \\
average_pause_dur   & 0.1392 & 0.099 & 1.411 & 0.159 \\
freq_pause          & 0.0220 & 0.018 & 1.248 & 0.213 \\
speech_rate         & -0.0140 & 0.025 & -0.563 & 0.574 \\
cons_correct        & -0.4647 & 0.656 & -0.709 & 0.479 \\
vowels_correct      & -0.3328 & 0.434 & -0.767 & 0.443 \\
VarcoC              & -0.0003 & 0.000 & -0.900 & 0.369 \\
perVB               & 0.0029 & 0.003 & 1.028 & 0.305 \\
nVB                 & 0.0046 & 0.007 & 0.691 & 0.490 \\
\bottomrule
\end{tabular}
\end{table}


==> figures/5_feature_selection.tex <==
\begin{table}[h]
\caption{
Monolingual classification (F1-score)  \\
}
\label{tab:importance}
% \vspace{-2mm}
%\scriptsize
\centering
\resizebox{0.70\textwidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline
Features & English & Korean & Tamil & Average \\
\hline
MFCCs & 36.96 & 62.71 & 40.36 & 46.68 \\
MFCCs + All & 48.07 & 72.64 & 46.52 & 55.74  \\
\hline
\textbf{Selected (gain)} & \textbf{59.03} & \textbf{76.40} & \textbf{46.91} & \textbf{60.78} \\
\hline

\end{tabular}
}
\end{table}
% \begin{table}[h]
% \caption{
% Classification accuracy by importance scores  \\
% (mono-lingual)
% }
% \label{tab:praat}
% % \vspace{-2mm}
% %\scriptsize
% \centering
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c}
% \hline
% Importance & English & Korean & Tamil & Average \\
% \hline
% MFCC & 24.96 & 64.88 & 51.93 &   \\
% MFCC + All & 21.79 & 74.00 & 62.73  &  \\
% \hline
% weight & 30.05  & 74.38 & 63.27 & \\
% gain & 32.69 & 74.88 & 62.94 & \\
% cover & 30.93  & \textbf{75.25} & 62.72 & \\
% total gain & \textbf{33.04} & 74.38 & \textbf{63.85} &  \\
% total cover & 31.99 & 75.13 & 63.28 &  \\
% \hline

% \end{tabular}
% }
% \end{table}

==> figures/5_korean_importance.tex <==
\begin{table}[htbp]
\centering
\caption{Feature Importance (Korean)}
\label{tab:feature_importance}
\begin{tabular}{lllr}
\toprule
\textbf{Features} & \textbf{Feature Type} & \textbf{Feature Subtype} & \textbf{Importance} \\
\midrule
PRR                      & pronunciation  & phoneme accuracy  & 0.0671 \\
CRR            & pronunciation  & phoneme accuracy  & 0.0443 \\
Mean F0                    & prosody        & F0                & 0.0381 \\
Median F0                  & prosody        & F0                & 0.0374 \\
VRR         & pronunciation  & phoneme accuracy  & 0.0360 \\
speaking rate             & prosody        & fluency           & 0.0352 \\
CPP & voice quality  & voice quality     & 0.0348 \\
Median energy                  & prosody        & energy            & 0.0347 \\
nPVI-C                   & prosody        & rhythm            & 0.0334 \\
\# of vb.                      & voice quality  & voice quality     & 0.0331 \\
average pause dur      & prosody        & fluency           & 0.0324 \\
Minimum energy                & prosody        & energy            & 0.0323 \\
VarcoV                   & prosody        & rhythm            & 0.0318 \\
VSA$\square$                    & pronunciation  & vowel distortion  & 0.0311 \\
Maximum energy                & prosody        & energy            & 0.0308 \\
VAI                      & pronunciation  & vowel distortion  & 0.0308 \\
articulation rate       & prosody        & fluency           & 0.0305 \\
shimmer             & voice quality  & voice quality     & 0.0304 \\
std. energy                   & prosody        & energy            & 0.0304 \\
F2-Ratio                       & pronunciation  & vowel distortion  & 0.0302 \\
percentage of vb.                    & voice quality  & voice quality     & 0.0302 \\
Maximum F0             & prosody        & F0                & 0.0301 \\
Minimum F0               & prosody        & F0                & 0.0300 \\
\%V                      & prosody        & rhythm            & 0.0300 \\
jitter              & voice quality  & voice quality     & 0.0298 \\
Mean energy                 & prosody        & energy            & 0.0295 \\
FCR                      & pronunciation  & vowel distortion  & 0.0291 \\
\# of pauses              & prosody        & fluency           & 0.0291 \\
VSA$\triangle$                    & pronunciation  & vowel distortion  & 0.0289 \\
APQ              & voice quality  & voice quality     & 0.0286 \\
\bottomrule
\end{tabular}
\end{table}

==> figures/5_method.tex <==
 \begin{figure*}
  \centering
\includegraphics[width=0.8\textwidth]{figures/TASLP_figure-final2.pdf}
  \caption{Workflow of automatic severity classification. SL denotes severity level.}
  \label{fig:overview2} 
\end{figure*}

==> figures/5_ssnce_importance.tex <==
\begin{table}[htbp]
\centering
\caption{Feature Importance (Tamil)}
\label{tab:feature_importance}
\begin{tabular}{lllr}
\toprule
\textbf{Features} & \textbf{Feature Type} & \textbf{Feature Subtype} & \textbf{Importance} \\
\midrule
Median F0               & prosody        & F0                & 0.1048 \\
PRR                     & pronunciation  & phoneme accuracy  & 0.0706 \\
CRR           & pronunciation  & phoneme accuracy  & 0.0479 \\
Mean F0                  & prosody        & F0                & 0.0510 \\
Minimum energy                & prosody        & energy            & 0.0419 \\
std. F0                    & prosody        & F0                & 0.0427 \\
std. energy                     & prosody        & energy            & 0.0405 \\
maximum F0                & prosody        & F0                & 0.0395 \\
Mean energy                    & prosody        & energy            & 0.0394 \\
CPP & voice quality  & voice quality     & 0.0385 \\
\%V                       & prosody        & rhythm            & 0.0377 \\
VRR         & pronunciation  & phoneme accuracy  & 0.0369 \\
nPVIC                   & prosody        & rhythm            & 0.0325 \\
speaking rate            & prosody        & fluency           & 0.0301 \\
articulation rate       & prosody        & fluency           & 0.0304 \\
Minimum F0              & prosody        & F0                & 0.0318 \\
Maximum energy               & prosody        & energy            & 0.0306 \\
VarcoC                   & prosody        & rhythm            & 0.0345 \\
nPVIV                   & prosody        & rhythm            & 0.0345 \\
F2-Ratio                     & pronunciation  & vowel distortion  & 0.0346 \\
VSA$\square$                     & pronunciation  & vowel distortion  & 0.0343 \\
VSA$\triangle$                   & pronunciation  & vowel distortion  & 0.0297 \\
VarcoV                   & prosody        & rhythm            & 0.0297 \\
FCR                      & pronunciation  & vowel distortion  & 0.0270 \\
VAI                      & pronunciation  & vowel distortion  & 0.0289 \\
\bottomrule
\end{tabular}
\end{table}

==> figures/5_tabular_example.tex <==
\begin{table}[h]
\caption{
Tabular for the proposed method
}
\label{tbl:table_example}

% \scriptsize
\centering
\resizebox{0.5\textwidth}{!}
{

\begin{tabular}{cccc}
\hline

Language & PCT & max F0 & APQ \\
\hline
English & O & N/A & N/A \\
Korean & O & O & N/A \\
Tamil & O & O & O \\
\hline

\end{tabular}

}
\end{table}

==> figures/5_vowel_distortion.tex <==
\begin{figure*}[h]
 \centering
 % \begin{subfig}{\textwidth} 
  \centering
\includegraphics[width=0.8\textwidth]{figures/5_vowel_space.pdf}
  \caption{Barplot of Vowel Distortion features.}
  \label{fig:vd}
 % \end{subfig}
 \end{figure*}

==> figures/6_classification.tex <==
\begin{table}[h]
\caption{
Cross-lingual classification (F1-score)
}
\label{tab:multiclassification}
% \vspace{-2mm}
%\scriptsize
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline
Experiment & English & Korean & Tamil & Average \\
\hline
%MFCC & 36.89 & 56.88 & 51.58 & 53.21  \\
% (1) All & 34.32 & 71.38 & 62.78 & 65.27\\
% \hline
% (2) Language-specific & 44.32 & 74.88 & 62.94 & 68.35\\
% (3) Language-independent & \textbf{47.70} & 69.38 & 61.04 & 64.77\\
% \hline
% (4) Union & 33.84 & 72.50 & 65.91 &56.90 \\
% \hline
% (5) Proposed  & 43.70 &\textbf{75.13} &\textbf{63.99} &\textbf{68.68} \\
% \hline
MFCCs & 60.66 & 59.64 & 38.78 & 53.03 \\
MFCCs + All & 66.99 & 72.47 & \textbf{55.75} & 65.07 \\
\hline
Intersection & 69.14 & 73.56 & 50.85 & 64.52 \\
Union & \textbf{71.96} & 72.76 & 55.48 & 66.74 \\
\textbf{Proposed}  & 69.46 & \textbf{78.13} & 53.84 & \textbf{67.14} \\
\hline
\end{tabular}
}
\end{table}

% \begin{table}[h]
% \caption{
% Classification accuracy by importance scores  \\
% (mono-lingual)
% }
% \label{tab:praat}
% % \vspace{-2mm}
% %\scriptsize
% \centering
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c}
% \hline
% Importance & English & Korean & Tamil & Average \\
% \hline
% MFCC & 24.96 & 64.88 & 51.93 &   \\
% MFCC + All & 21.79 & 74.00 & 62.73  &  \\
% \hline
% weight & 30.05  & 74.38 & 63.27 & \\
% gain & 32.69 & 74.88 & 62.94 & \\
% cover & 30.93  & 75.25 & 62.72 & \\
% total gain & 33.04 & 74.38 & 63.85 &  \\
% total cover & 31.99 & 75.13 & 63.28 &  \\
% \hline

% \end{tabular}
% }
% \end{table}


==> figures/7_comparison.tex <==
\begin{table}[h]
\caption{
Comparison with mono-lingual classifiers  \\
}
\label{tab:compare}
% \vspace{-2mm}
%\scriptsize
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Language & Mono-lingual & Proposed & Relative Increase \\
\hline
English & 59.03 & \textbf{69.46} & 17.67 \\
Korean & 76.39 & \textbf{78.13} & 2.28  \\
Tamil & 49.95 & \textbf{53.84} &  7.79 \\
\hline
Average & 61.79 & \textbf{67.14} & 8.66 \\ 
\hline

\end{tabular}
}
\end{table}


==> figures/ablation.tex <==
\begin{table}[h]
\caption{
Ablation study on hyperparameters $\alpha$ and $e$.
}
\label{tab:ablation}
\centering
\resizebox{0.5\textwidth}{!}
{
\begin{tabular}{c|c|c|c|c}

\hline
Accuracy & $\alpha=1.0$ & $\alpha=0.1$ & $\alpha=0.01$ & $\alpha=0.001$ \\
\hline
$e=0$  & 60.51 & 60.69 & 56.21 & 54.94 \\
\hline
$e=10$ & 61.82 & 63.12 & 57.14 & 57.00 \\
\hline
$e=20$ & 54.77 & 64.69 & 59.84 & 61.27 \\
\hline
$e=30$ & 57.74 & \textbf{65.52} & 60.10 & 62.72 \\
\hline
$e=40$ & 55.47 & 60.11 & 62.00 & 57.96 \\
\hline
\hline
PER & $\alpha=1.0$ & $\alpha=0.1$ & $\alpha=0.01$ & $\alpha=0.001$ \\
\hline
$e=0$  & 17.50 & 21.86 & 88.49 & 96.91 \\
\hline
$e=10$ & 14.83 & 22.37 & 82.59 & 96.49 \\
\hline
$e=20$ & 16.66 & 18.10 & 31.12 & 90.08 \\
\hline
$e=30$ & 15.87 & 17.72 & 23.10 & 74.54 \\
\hline
$e=40$ & 15.41 & 15.95 & 20.45 & 56.24 \\
\hline
\end{tabular}
}

\vspace{-1em}

\end{table}


%

==> figures/alignment.tex <==
\begin{table}[h]
\captionsetup{justification=centering}
\caption{Alignment for phoneme correctness extraction}
\label{tab:alignment}
\centering
\resizebox{0.40\textwidth}{!}{
\begin{tabular}{c}
\hline\hline
Canonical phoneme sequence \\
\hline
% \hline
HH  IY  W  IH  L  AH  L  AW  AH  *  R  EH  L  AY \\
\hline
\hline
Decoded phoneme sequence \\
\hline
SH  IY  W  AO  L  AH  L  AW  AE  N  L  IY  *  AY\\
\hline
\hline
\end{tabular}
}
\end{table}

==> figures/confusion_matrix.tex <==
\begin{figure*}[t!] % t: top, b: bottom, h: here
\centering
\subfloat[English_All]{\includegraphics[width=0.23\textwidth]{figures/multi_e_mfccALL_100.pdf}}
\subfloat[English_Intersection]{\includegraphics[width=0.23\textwidth]{figures/e_gain_C_100.pdf}}
\subfloat[English_Union]{\includegraphics[width=0.23\textwidth]{figures/e_gain_D_400.pdf}}
\subfloat[English_Proposed]{\includegraphics[width=0.23\textwidth]{figures/e_gain_E_100.pdf}}

\subfloat[Korean_All]{\includegraphics[width=0.23\textwidth]{figures/multi_k_mfccALL_100.pdf}}
\subfloat[Korean_Intersection]{\includegraphics[width=0.23\textwidth]{figures/k_gain_C_100.pdf}}
\subfloat[Korean_Union]{\includegraphics[width=0.23\textwidth]{figures/k_gain_D_400.pdf}}
\subfloat[Korean_Proposed]{\includegraphics[width=0.23\textwidth]{figures/k_gain_E_100.pdf}}

\subfloat[Tamil_All]{\includegraphics[width=0.23\textwidth]{figures/multi_ta_mfccALL_100.pdf}}
\subfloat[Tamil_Intersection]{\includegraphics[width=0.23\textwidth]{figures/t_gain_C_100.pdf}}
\subfloat[Tamil_Union]{\includegraphics[width=0.23\textwidth]{figures/t_gain_D_400.pdf}}
\subfloat[Tamil_Proposed]{\includegraphics[width=0.23\textwidth]{figures/t_gain_E_100.pdf}}
\caption{Confusion Matrix for MFCCs+ALL, Intersection, Union, and Proposed experiments}
\label{fig:confusion}
\end{figure*}


==> figures/diagram.tex <==
\begin{figure*}[t!] % t: top, b: bottom, h: here
\centering
\includegraphics[width=1\textwidth,height=5cm]{figures/dysarthria-gop.pdf}
\caption{Overview of the improved GoP with UQ methods.}
\vspace{-1em}
\label{fig:diagram}
\end{figure*}

==> figures/method-2.tex <==
\begin{figure}[h] %%% t: top, b: bottom, h: here
\centering
\includegraphics[width=0.75\columnwidth]{figures/method-fig.pdf}
\caption{
Example of Deep learning-based approaches \citep{yeo2023automatic}.
}
\label{figs:method-2}
\end{figure}

==> figures/method-5.tex <==
\begin{figure*}[t] % t: top, b: bottom, h: here
\centering
\includegraphics[width=\textwidth]{figures/TASLP-figure1.pdf}
\caption{Overview of the proposed method.}
\label{fig:diagram}
\end{figure*}

==> figures/mono_ablation.tex <==
\begin{table}[t]
\caption{Monolingual classification results without distance-based features. Best performances are indicated in bold.}
\label{tab:xgboost_performance}
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
Feature Set & English & Korean & Tamil & Average \\ 
\midrule
MFCC & 53.12 & 67.37 & 54.48 & 57.66 \\
eGemaps& 36.60 & 75.41 & 52.75 & 54.92 \\
Hand-crafted-a & 52.62 & 78.75 & 61.93 & 64.43 \\
\textbf{Hand-crafted-b} & \textbf{54.03} & \textbf{79.47}  & \textbf{68.83}  & \textbf{67.44}  \\
\bottomrule
\end{tabular}%
}\label{tab:monolingual-ablation}
\end{table}

%\begin{table}[htbp]
% \caption{\fix{Monolingual} classification results without distance-based features}
% \label{tab:xgboost_performance}
% \centering
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% Feature Set & English & Korean & Tamil & Average \\ 
% \midrule
% MFCC & 52.68 & 64.60 & 55.10 & 57.46 \\
% eGemaps & 34.49 & 74.05 & 52.83 & 53.79 \\
% Hand-crafted-a & 51.90 & 78.43 & 55.00 & 61.78 \\
% \textbf{Hand-crafted-b} & \textbf{52.62} & \textbf{79.35} & \textbf{68.56} & \textbf{66.84} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


==> figures/multi_ablation.tex <==
\begin{table}[t]
\caption{Multilingual classification without distance-based features. Best performances are indicated in bold.}
\label{tab:xgboost_classification}
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
Feature Set & English & Korean & Tamil & Average \\ 
\midrule
MFCC & 61.73 & 69.18 & 51.90 & 60.94 \\
eGemaps & \textbf{68.26} & 68.07 & 55.86 & 64.06 \\
Intersection & 66.84 & 71.82 & \textbf{71.91} & 70.19 \\
Union & 56.66 & 79.77 & 67.22 & 67.88 \\
Proposed & 61.23 & \textbf{81.42} & 69.02 & \textbf{70.56} \\
\bottomrule
\end{tabular}%
\label{tab:multilingual-ablation}}
\end{table}


==> figures/regularization.tex <==
\begin{figure}[h] %%% t: top, b: bottom, h: here
\centering
\includegraphics[width=0.9\columnwidth]{figures/loss.pdf}
\caption{
Classification loss $\mathcal{L}_\texttt{CE}$ and ASR loss $\mathcal{L}_\texttt{CTC}$ on validation set.
$\alpha=0$ denotes the STL case when we use the $\mathcal{L}_\texttt{CE}$ only.
% For the MTL case, we enable $\mathcal{L}_\texttt{CE}$ after $e$ epochs of training.
}
\label{fig:regularization}
\end{figure}

==> figures/representation.tex <==
\begin{figure}[t!] %%% t: top, b: bottom, h: here
\centering
\vspace{-2em}
\subfloat[Trained with MTL,\\color-coded with severity.]{\includegraphics[width=0.43\columnwidth]{figures/repr-severity-MTL.pdf}}
\subfloat[Trained with STL,\\color-coded with severity.]{\includegraphics[width=0.43\columnwidth]{figures/repr-severity-STL.pdf}}\\
\vspace{-1em}
\subfloat[Trained with MTL,\\color-coded with setence.]{\includegraphics[width=0.43\columnwidth]{figures/repr-script-MTL.pdf}}
\subfloat[Trained with STL,\\color-coded with setence.]{\includegraphics[width=0.43\columnwidth]{figures/repr-script-STL.pdf}}
\caption{
Averaged representation $\overline{\mathbf{h}}$ of the training set samples.
$0$ to $4$ refers to severity levels, starting from healthy to severe.
$s$ in $s1...s2$ refers to sentences.
% Two cases are considered: (1) classification and ASR jointly trained (MTL) and (2) trained with classification only (STL).
% The training set contains five level of severity and five reference text.
}
\vspace{-1em}
\label{figs:representation}
\end{figure}

==> figures/results.tex <==
\begin{table}[t]
\caption{
Classification performance compared to the baselines.
}
\label{tab:results}
\centering
\resizebox{0.7\textwidth}{!}
{

\begin{tabular}{c|c|c|c|c|c}
\hline
Input & Classifier & Accuracy & Precision & Recall & F1-score\\
\hline
\multirow{3}{*}{eGeMAPS}
& SVM & 55.01 & 53.89 & 53.27 & 52.28 \\
& MLP & 50.79 & 44.46 & 48.60 & 46.58 \\
& XGBoost & 52.20 & 55.07 & 50.85 & 50.61 \\
\hline
\multirow{3}{*}{\shortstack{Hand-crafted\\ features}}
& SVM & 61.02 & 64.19 & 63.19 & 62.41 \\
& MLP & 55.74 & 60.06 & 60.34  & 58.85 \\
& XGBoost & 55.72 & 61.14 & 56.21 & 56.16 \\
\hline
\multirow{3}{*}{\shortstack{eGeMaps\\ + Hand-crafted \\ features}}
& SVM & 57.83 & 58.83 & 57.59 & 56.65 \\
& MLP & 50.21 & 48.40 & 47.31 & 46.76 \\
& XGBoost & 56.29 & 62.29 & 56.23 & 56.68 \\
\hline
\multirow{2}{*}{Raw audio} 
& STL & 61.02 & 64.09 & 57.93 & 57.13 \\
& \textbf{MTL} & \textbf{65.52} & \textbf{66.47} & \textbf{64.86} & \textbf{63.19} \\
\hline
\end{tabular}


% \begin{tabular}{c|c|c|c|c|c}
% \hline
% Input & Classifier & Accuracy & Precision & Recall & F1-score\\
% \hline
% \multirow{3}{*}{eGeMAPS} & SVM & 51.11 & 51.24 & 55.20 & 52.58\\
% & MLP & 42.22 & 40.09 & 46.80 & 42.12 \\
% & XGBoost & 52.78 & 53.33 & 55.07 & 53.53 \\
% \hline
% \multirow{3}{*}{\shortstack{Linguistic\\ features}} & SVM & 49.44 & 53.44 &  57.20 & 54.36 \\
% & MLP & 41.67 & 46.26 & 52.40  & 48.75 \\
% & XGBoost & 54.44 & 54.24 & 63.53 & 56.66 \\
% \hline
% \multirow{3}{*}{\shortstack{eGeMaps\\ + Ling.}} & SVM & 48.33 & 51.77 & 55.13 & 53.26\\
% & MLP & 40.56 & 43.26 & 47.13 &  44.62\\
% & XGBoost & 57.78 & 58.18 &\textbf{64.67} & 60.07 \\
% \hline
% \multirow{2}{*}{Raw audio} 
% & STL & 55.00 & 59.77 & 57.47 & 58.09 \\
% & \textbf{MTL} & \textbf{60.55} & \textbf{62.29} & 64.33 & \textbf{62.37} \\
% \hline
% \end{tabular}
}
\vspace{-1em}
\end{table}


%

==> figures/selected_features_cover.tex <==
\begin{table*}[h]
\caption{Optimal feature sets}
\label{tab:cover}
\centering

\resizebox{0.9\textwidth}{!}{

\begin{tabular}{c|c|c|c}

\hline
\multirow{2}{*}{Category} & \multicolumn{3}{c}{Languages} \\
\cline{2-4}
 & English & Korean & Tamil \\
\hline
voice quality & HNR & - &  APQ, shimmer, degree of voice breaks \\
\hline
phoneme correctness & \textbf{PCT} & \textbf{PCT} & PCC, \textbf{PCT} \\
\hline
vowel distortion & - & - & VSA$\square$, VAI, F2-ratio \\
\hline
speech rate & - & pause duration, phone ratio  & - \\
\hline
pitch & - & \underline{max} F0 & mean/min/\underline{max}/std F0 \\
\hline
loudness & \underline{min}/\underline{max} energy & \underline{std} energy & mean/\underline{min}/\underline{max}/\underline{std} energy \\
\hline
rhythm & deltaV, deltaC & - & VarcoV, nPVIV \\
\hline

% \hline
% \multirow{2}{*}{Voice quality} & Glottal flow & jitter, shimmer, PPQ, APQ, HNR \\
% \cline{2-3}
% & Phonation & \# of voice breaks, \% of voice breaks \\
% \hline

% \multirow{2}{*}{Pronunciation} & Phoneme correctness & PCC, PCV, PCP \\
% \cline{2-3}
% & Vowel distortion & triangular VSA, quadrilateral VSA, FCR, VAI, F2-Ratio \\
% \hline

% \multirow{5}{*}{Prosody} 
% & Speech rate & speaking rate, articulation rate, number of pauses, pause duration, phone ratio \\
% \cline{2-3}
% & Pitch & mean, median, std, min, max, range of F0 \\
% \cline{2-3}
% & Intensity & mean, median, std, min, max, range of energy \\
% \cline{2-3}
% & Rhythm & \%V, deltaV/C, VarcoV/C, rPVIV/C, nPVIV/C \\
% \cline{2-3}
% \hline

\end{tabular}
}
\end{table*}

==> figures/stats_tbl.tex <==
\begin{table*}[t]
\caption{Mean values of acoustic measurements }
\label{tab:analysis1}
\centering
\resizebox{0.9\textwidth}{!}{

\begin{tabular}{cc|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}

\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Measurements}} & \multicolumn{5}{c|}{English} & \multicolumn{5}{c|}{Korean} & \multicolumn{5}{c}{Tamil} \\
\cline{3-17}
& & healthy & dys & mild & moderate & severe & healthy & dys & mild & moderate & severe & healthy & dys & mild & moderate & severe \\
\cline{1-17}
\multirow{7}{*}{Voice quality} & jitter & 2.31 & 2.33 & 2.37 & 1.64 & 2.79 & 1.72 & 1.83 & 1.59 & 1.95 & 1.88 & 1.47 & 1.23 & 1.23 & 1.18 & 1.37\\
& shimmer & 12.07 & 8.99 & 9.97 & 5.97 & 9.46 & 7.53 & 7.73 & 6.91 & 8.28 & 7.29 & 8.07 & 7.14 & 7.15 & 7.00 & 7.57\\
& PPQ & 1.11 & 1.14 & 1.14 & 0.70 & 1.52 & 0.78 & 0.80 & 0.68 & 0.86 & 0.83 & 0.68 & 0.59 & 0.60 & 0.54 & 0.73\\
& APQ & 6.94 & 4.94 & 5.63 & 2.85 & 5.21 & 3.25 & 3.64 & 3.16 & 3.99 & 3.21 & 3.64 & 3.48 & 3.39 & 3.34 & 4.14\\
& HNR & 9.95 & 12.94 & 11.39 & 18.03 & 11.96  & 16.27 & 16.18 & 16.82 & 15.80 & 16.31 & 14.01 & 15.63 & 15.72 & 15.67 & 15.26\\
& number of VBs & 6.83 & 9.04 & 6.86 & 9.85 & 12.84 & 6.51 & 10.87 &  9.47 & 11.06 & 14.36 & 4.05 & 3.75 &  3.73 & 3.81 & 3.61\\
& degree of VBs & 16.49 & 21.60 & 19.04 & 25.94 & 23.33 & 13.82 & 30.29 & 1.59 & 1.95 & 1.88 & 19.93  & 19.73 & 18.26 & 20.79 & 19.64 \\
\cline{1-17}
\multirow{8}{*}{Pronunciation} &  \textbf{PCC} &  \textbf{95.93} &  \textbf{80.44} & 94.25 & 71.08 & 59.76 &  \textbf{97.53} & \textbf{57.74} & 83.47 & 50.92 & 12.18 & \textbf{93.17} & \textbf{55.22} & 70.42 & 53.08 & 26.90 \\
& \textbf{PCV} & \textbf{94.51} & \textbf{77.06} & 93.16 & 64.19 & 54.58 & \textbf{99.04} & \textbf{69.44} & 88.90 & 65.96 & 25.34 & \textbf{91.52} & \textbf{52.55} &  65.90 & 50.16 & 29.35 \\
& \textbf{PCP} & \textbf{95.28} & \textbf{78.90} & 93.79 & 67.93 & 57.35 & \textbf{98.20} & \textbf{62.84} & 85.85 & 57.48 & 17.90 & \textbf{92.63} & \textbf{54.47} & 69.08 & 52.28 & 27.68 \\
\cline{2-17}
& \textbf{triangular VSA} & \textbf{109791} & \textbf{84913} & 110459 & 50541 & 60574 & \textbf{199831} & \textbf{111081} & 149994 & 97226 & 62400 & \textbf{207104} & \textbf{82208} & 97715 & 85328 &35626 \\
& \textbf{quadrilateral VSA} & \textbf{162175} & \textbf{130753} & 169389 & 102766 & 74430 & \textbf{202496} & \textbf{110192} & 149031 & 95282 & 67779 & \textbf{240516} & \textbf{95325} & 114907 & 97589 & 42085 \\
& \textbf{FCR} & \textbf{1.28} & \textbf{1.33} & 1.25 & 1.38 & 1.46 & \textbf{1.35} & \textbf{1.60} & 1.40 & 1.67 & 1.85 & \textbf{1.15} & \textbf{1.46} & 1.37 & 1.47 & 1.64\\
& \textbf{VAI} & \textbf{0.80} & \textbf{0.76} & 0.81 & 0.73 & 0.69 & \textbf{0.78} & \textbf{0.66} & 0.75 & 0.63 & 0.55 & \textbf{0.89} & \textbf{0.70} & 0.74 & 0.70 & 0.63 \\
& \textbf{F2-Ratio} & \textbf{1.36} & \textbf{1.37} & 1.43 & 1.31 & 1.29 & \textbf{1.56} & \textbf{1.34} & 1.55 & 1.25 & 1.12 & \textbf{2.13} & \textbf{1.55} & 1.67 & 1.53 & 1.31\\
\cline{1-17}
\multirow{25}{*}{Prosody} & speaking rate & 2.96 & 2.76 & 2.80 & 2.49 & 2.90 & 3.41 & 2.41 & 2.79 & 2.33 & 1.59 & 2.49 & 2.56 & 2.72 & 2.43 & 2.62\\
& \textbf{articulation rate} & \textbf{6.39} & \textbf{5.69} &  6.11 & 4.78 & 5.57 & \textbf{5.67} & \textbf{5.33} & 5.20 & 5.33 & 5.74 & \textbf{5.46} & \textbf{4.36} & 4.57 & 4.31 & 4.04\\
& \textbf{number of pauses} & \textbf{1.40} & \textbf{2.89} & 1.65 & 4.90 & 3.80 & \textbf{1.49} & \textbf{5.23} & 3.49 & 5.73 & 8.13 & \textbf{2.14} & \textbf{2.32} & 2.25 & 2.31 & 2.48 \\
& pause duration & 2.44 & 3.25 & 2.58 & 4.18 & 3.87 & 1.52 & 4.90 & 2.93 & 5.00 & 10.90 & 1.85 & 1.38 &  1.37 & 1.47 & 1.11 \\
& phone ratio & 0.46 & 0.49 & 0.46 & 0.52 & 0.52 & 0.60 & 0.47 & 0.54 & 0.45 & 0.32 & 0.46 & 0.59 & 0.69 & 0.57 & 0.66\\
\cline{2-17}
& F0 mean & 60.03 & 79.44 & 69.53 & 87.45 & 93.21 & 98.57 & 83.76 & 91.55 & 80.91 & 74.39 & 88.44 & 123.51 & 110.04 & 124.31 & 148.94\\
% & F0 median & 158.57 & 0 & 185.68 & 166.09 & 155.01 & 188.18 & 0 & 191.71 & 188.77 & 227.05 & 294.13 & 0 & 193.03 & 230.86 & 234.81\\
& \textbf{F0 std} & \textbf{90.10} & \textbf{94.77} & 96.06 & 90.70 & 95.43 & \textbf{95.64} & \textbf{99.80} & 97.76 & 99.29 & 109.38 & \textbf{106.23} & \textbf{218.21} & 95.52 & 114.46 & 112.01\\
& F0 min & 106.53 & 101.76 & 112.40 & 91.98 & 87.94 & 102.17 & 102.22 & 103.20 & 102.50 & 97.36 & 149.14 & 107.46 & 141.44 & 157.15 & 153.33\\
& F0 max & 420.77 & 410.33 & 394.67 & 401.32 & 449.69 & 261.97 & 405.76 & 339.47 & 436.04 & 450.51 & 311.67 & 151.08 & 258.36 & 307.79 & 285.48\\
& F0 range & 314.23 & 308.57 & 282.27 & 309.35 & 361.75 & 159.80 & 303.54 & 236.27 & 333.54 & 353.15 & 162.53 & 136.06 & 116.92 & 150.64 & 132.15\\
\cline{2-17}
& energy mean & 53.02 & 58.38 & 56.36 & 57.50 & 63.24 & 51.64 & 48.44 & 49.52 & 48.35 & 45.46 & 40.21 & 42.32 & 42.03 & 40.68 & 48.45\\
% & energy median & 49.29 & 14.01 & 51.22 & 58.56 & 62.10 & 58.98 & 0 & 53.21 & 48.80 & 43.98 & 39.93 & 0 & 46.92 & 44.72 & 55.10\\
& energy std & 12.26 & 14.01 & 13.19 & 15.96 & 14.10 & 19.34 & 16.23 & 17.48 & 15.64 & 15.45 & 22.07 & 47.04 & 17.57 & 17.91 & 17.40\\
& \textbf{energy min} & \textbf{39.92} & \textbf{40.52} & 41.56 & 34.25 & 43.50 & \textbf{15.17} & \textbf{16.62} & 15.89 & 17.16 & 15.97 & \textbf{12.63} & \textbf{17.72} & 12.48 & 11.98 & 13.42\\
& energy max & 77.50 & 83.44 & 81.96 & 82.95 & 86.84 & 77.24 & 77.01 &  75.84 & 77.10 & 80.36 & 73.76 & 66.99 & 66.45 & 66.29 & 70.57\\
& energy range & 37.58 & 42.91 & 40.41 & 48.70 & 43.34 & 62.07 & 60.39 & 59.95 & 59.94 & 64.39 & 61.14 & 66.99 & 53.97 & 54.30 & 57.15\\
\cline{2-17}
& \textbf{\%V} & \textbf{41.72} & \textbf{43.56} & 41.45 & 45.65 & 46.18 & \textbf{84.07} & \textbf{87.46} & 85.91 & 87.70 & 91.18 & \textbf{47.09} & \textbf{55.27} &  54.78 & 54.28 & 59.68\\
& \textbf{deltaV} & \textbf{60.70} & \textbf{93.36} & 63.19 & 131.37 & 124.19 & \textbf{475.79} & \textbf{1215.04} & 787.42 & 1153.54 & 2971.46 & \textbf{62.06} & \textbf{76.47} & 71.92 & 76.44 & 87.18\\
& \textbf{deltaC} & \textbf{73.28} & \textbf{106.23} & 73.72 & 133.00 & 151.02 & \textbf{53.38} & \textbf{150.04} & 103.58 & 153.93 & 280.42 & \textbf{59.79} & \textbf{66.69} & 65.60 & 69.65 & 59.37\\
& VarcoV & 53.18 & 50.87 & 52.66 & 48.02 & 49.52 & 90.88 & 94.92 & 90.45 & 92.84 & 121.45 & 52.51 & 51.76 &  47.64 & 54.26 & 53.02\\
& \textbf{VarcoC} & \textbf{50.89} & \textbf{54.82} & 49.86 & 57.54 & 62.76 & \textbf{45.04} & \textbf{76.40} & 60.47 & 78.29 & 117.91 & \textbf{50.55} & \textbf{58.03} & 54.30 & 61.05 & 56.71\\
& \textbf{rPVIV} & \textbf{66.20} & \textbf{102.61} & 67.47 & 145.11 & 139.97 & \textbf{454.49} & \textbf{1101.09} & 758.96 & 1083.72 & 2324.55 & \textbf{73.08} & \textbf{87.19} & 81.13 & 87.78 & 99.35\\
& \textbf{rPVIC} & \textbf{81.85} & \textbf{115.28} & 77.76 & 141.92 & 170.44 & \textbf{66.88} & \textbf{174.43} & 120.21 & 179.87 & 321.56 & \textbf{72.74} & \textbf{79.73} & 78.69 & 83.05 & 71.09\\
& nPVIV & 55.85 & 54.00 & 55.22 & 52.42 & 52.79 & 84.37 & 91.71 & 86.47 & 92.23 & 105.95 & 60.27 & 58.18 & 52.27 & 61.48 & 61.00 \\
& \textbf{nPVIC} & \textbf{56.89} & \textbf{58.37} & 53.14 & 63.30 & 65.06 & \textbf{53.44} & \textbf{79.91} & 55.58 & 82.73 & 107.32 & \textbf{59.81} & \textbf{66.65} & 62.57 & 69.52 & 65.52\\
\hline

\end{tabular} 
}
\end{table*}

